On the Approximation Power of Two-Layer Networks of Random ReLUs

This paper considers the following question: how well can depth-two ReLU networks with randomly initialized bottom-level weights represent smooth functions? We give near-matching upper- and lower-bounds for $L_2$-approximation in terms of the Lipschitz constant, the desired accuracy, and the dimension of the problem, as well as similar results in terms of Sobolev norms. Our positive results employ tools from harmonic analysis and ridgelet representation theory, while our lower-bounds are based on (robust versions of) dimensionality arguments.

==> Lipschitz.tex <==
%

\section{Proofs of Upper \& Lower Bounds for Lipschitz Functions in $\fnmeas{\intvl^d}$ }\label{section:proofs-Lipschitz}



In this appendix, we present the proofs of the main propositions for the representational power of RBL ReLU Networks in the class of Lipschitz functions in $\fnmeas{\intvl^d}$.

\subsection{Trigonometric Polynomial Approximation for Lipschitz Functions}\label{ssec:trig-lipschitz-approx}

We show that all $L$-Lipschitz functions over $\intvl^d$ can be approximated by bounded-degree trigonometric polynomials with small coefficients.

\begin{lemma}[Approximating Lipschitz Functions with Bounded-Degree Trig Polynomials]\label{lemma:trig-lipschitz-approx}
	Fix some $L, \eps > 0$ with $\frac{L}{\eps} \geq 1$ and consider any function $f: \R^d \to \R$ with $f \in L^2([-1, 1]^d)$, $\norm[\lip]{f} \leq L$, and $\abs{\EE[\bx]{f(\bx)}} \leq L$. 
	Then, there exists a bounded-degree trigonometric polynomial \[P(x) = \sum_{K \in \mathcal{K}_{k,d}} \beta_K T_{K}\paren{\frac{x}{2}} \]
	for $k = \frac{L}{\eps}$ such that 
	$\norm[\intvl^d]{f - P} \leq \eps.$
	For all $K$, $\abs{\beta_K} \leq L$. \end{lemma}

\begin{proof}	
	We give a low-degree trigonometric polynomial approximation for $f$ by showing that high-degree coefficients of the trigonometric expansion are very small. We do so by taking term-by-term derivatives, requiring that $f$ satisfy periodic boundary conditions (see Lemma \ref{lemma:trig-expansion-deriv}), which our statement does not guarantee. We can work around this requirement with a reduction described below. 
	
	Roughly, the argument proceeds as follows:
	\begin{enumerate}
		\item\label{step:1} We define $\bar{f}: \intv^d \to \R$ to be a rescaling and shift of $f$ so that its domain is the cube $\intv^d$. That is, $\bar{f}(x) = f(2x - \vec{1})$ and $f(x) = \bar{f}\paren{\frac{1}{2}(x + \vec{1})}$. %
		Then it holds that $\norm[\lip]{\bar{f}} \leq 2L$ and $\abs{\EE[\bx \sim\intv^d]{\bar{f}(\bx)}} = \abs{\EE[\bx\sim \intvl^d]{{f}(\bx)}} \leq L$. 
		\item\label{step:2} We define $\tilde{f}: \intvl^d \to \R$ by reflecting $\bar{f}$ across orthants as follows: $\tilde{f}(x) = \bar{f}(\sign{x} \odot x)$, where $\sign{x} := (\sign{x_1}, \dots, \sign{x_d})$ and $\odot$ represents element-wise multiplication. The function $\tilde{f}$ is $2L$-Lipschitz, has periodic boundary conditions, and has $\abs{\EE[\bx\sim \intvl^d]{\tilde{f}(\bx)}} = \abs{\EE[\bx\sim \intv^d]{\bar{f}(\bx)}} \leq L$.
		\item\label{step:3} We find a low-degree trigonometric polynomial $\tilde{P}$ that $\eps$-approximates $\tilde{f}$ over $\intvl^d$.
		\item\label{step:4} Then, $\tilde{P}$ $\eps$-approximates $\tilde{f}$ in at least one of the $2^d$ unit cubes contained in each orthant of $\intvl^d$. Therefore, there exists some $w \in \flip^d$ such that $\bar{f}(x)$ is approximated by $\tilde{P}(w \odot x)$ on $\intv^d$.
		\item\label{step:5} By shifting and rescaling $\tilde{P}(w \odot x)$, we obtain a trigonometric polynomial $P$ that $\eps$-approximates $f$ on $\intvl^d$ as desired.
	\end{enumerate}
    
    \begin{figure}[h!]
    \centering
    	\ignore[true]{
		\begin{tikzpicture}[scale=0.9]  		
		\begin{scope}[scale=0.7]
 			\begin{axis}[domain=-1:1,y domain=-1:1, xlabel={$x_1$}, ylabel={$x_2$},zlabel={$f(x)$}]				
    				\addplot3[surf] {x * y^3};
  			\end{axis}
  		\end{scope}
  		\begin{scope}[xshift=8cm,scale=0.7]
 			\begin{axis}[domain=-1:1,y domain=-1:1, xlabel={$x_1$}, ylabel={$x_2$},zlabel={$\tilde{f}(x)$}]	
    				\addplot3[surf, domain=0:1, y domain=0:1] {(2*x - 1) * (2 * y - 1)^3};
				\addplot3[surf, domain=-1:0, y domain=0:1] {(-2*x - 1) * (2 * y - 1)^3};
				\addplot3[surf, domain=0:1, y domain=-1:0] {(2*x - 1) * (-2 * y - 1)^3};
				\addplot3[surf, domain=-1:0, y domain=-1:0] {(-2*x - 1) * (-2 * y - 1)^3};
  			\end{axis}
  		\end{scope}
  		\begin{scope}[xshift=8cm,yshift=-6cm,scale=0.7]
 			\begin{axis}[domain=-1:1,y domain=-1:1, xlabel={$x_1$}, ylabel={$x_2$},zlabel={$\tilde{P}(x)$}]	
    				\addplot3[surf] {0.132 *sqrt(2) * cos(pi * (deg(x)+deg(y)))+0.132 *sqrt(2) * cos(pi * (deg(x)-deg(y)))};
  			\end{axis}
  		\end{scope}
  		\begin{scope}[xshift=0cm,yshift=-6cm,scale=0.7]
 			\begin{axis}[domain=-1:1,y domain=-1:1, xlabel={$x_1$}, ylabel={$x_2$},zlabel={$P(x)$}]	
    				\addplot3[surf] {0.132 *sqrt(2) * cos(pi/2 * (deg(x+1)+deg(y+1)))+0.132 *sqrt(2) * cos(pi/2 * (deg(x)-deg(y)))};
  			\end{axis}
  		\end{scope}
  		\draw[thick,->] (5,2) to (7,2);
  		\draw (6,1.5) node {Step 1};
  		\draw (0,-0.25) node {(a)};
  		\draw (8,-0.25) node {(b)};
  		\draw (8,-6.25) node {(c)};
  		\draw (0,-6.25) node {(d)};
  		\draw[thick,->] (10,0) to (10,-2);
 		\draw (9.25,-1) node {Step 2};
  		%
  		\draw[thick,<-] (5,-4) to (7,-4);
		\draw (6,-4.5) node {Step 3};
  		\def\ytranspose{-0.2};
  		\draw (2.75,-0.4+\ytranspose) to[bend right] (2.75,-1+\ytranspose);
  		\draw (2.75,-1+\ytranspose) to[bend left]  (2.75,-1.6+\ytranspose);
  		\draw (2.25,-0.4+\ytranspose) to[bend right] (2.25,-1+\ytranspose);
  		\draw (2.25,-1+\ytranspose) to[bend left]  (2.25,-1.6+\ytranspose);
		\end{tikzpicture}
		}
		\caption{Visualizes the function transformations used to give an approximation of $f$ in Lemma \ref{lemma:trig-lipschitz-approx}. The original function $f$ is in (a), which is scaled and reflected to yield a function $\tilde{f}$ with periodic boundary conditions in (b), which is given a trigonometric polynomial approximation $\tilde{P}$ in (c), which is in turn scaled and shifted to obtain $P$ approximating $f$ in (d). \cs{Add the figure back when we're ready to hand in!}}
\end{figure}

	Steps (\ref{step:1}) and (\ref{step:2}) are immediate. We prove step (\ref{step:3}) by proving the existence of $\tilde{P}$.
	Because $\mathcal{T}$ is an orthonormal basis over $\fnmeas{[-1, 1]^d}$, we can express $\tilde{f}$ as 
	\[\tilde{f}(x) = \sum_{K \in \Z^d} \tilde{\alpha}_K T_K(x).\]
			
	To relate $\tilde{f}$ to its Lipschitz constant, we consider its derivatives.
	Because $f$ is differentiable, $\tilde{f}$ is also differentiable everywhere in $[-1, 1]^d$ except $S := \set{x \in \intvl^d: \ \exists \  i \in [d] \text{ s.t. } x_i = 0}$, where its partial derivatives are undefined because different reflections of $\bar{f}$ may give different partial derivatives at the same point. 
	However, we can safely assume that $\tilde{f}$ does indeed have partial derivatives defined everywhere due to a \href{http://www.tricki.org/article/To_make_a_function_nicer_without_changing_it_much_convolve_it_with_an_approximate_delta_function}{standard approximation argument}, which shows that we can approximate $\tilde{f}$ arbitrarily well by convolving it with an approximate delta function, while making this approximation differentiable. 
	\cs{Make this a little less sketchy\dots Option 1: Give some $f'' := f \star \text{Box}(\eps)$. Show that $f''$ is approximation of $f$, $f''$ is differentiable. $f''$ is Lipschitz. Maybe take $\eps$ to 0; maybe just keep $\eps$ small.}
	\rs{\url{http://arxiv.org/abs/math/0602051}}
	Because of the Lipschitzness of $f$ and the continuity of $\tilde{f}$, the partial derivatives assigned through this approximation are such that $\norm[2]{\nabla \tilde{f}(\bx)} \leq 2L$ for all $x \in S$.
	We thus have a clean expression for the expected squared gradient norm of $\tilde{f}$, which can be no more than $4L^2$. 
%
%
%
	\begin{align*}
		4L^2
		&\geq \EE[\bx \sim \intvl^d]{\norm[2]{\nabla \tilde{f}(\bx)}^2} = \sum_{i=1}^d \EE[\bx]{\paren{\pderiv{\tilde{f}(\bx)}{\bx_i}}^2} = \sum_{i=1}^d \EE[\bx]{\paren{\sum_{K \in \Z^d} \tilde{\alpha}_K \pderiv{T_K(\bx)}{\bx_i}}^2}  \stepcounter{equation}\tag{\theequation}\label{line:nnn} \\
		&= \sum_{i=1}^d \sum_{K \in \Z^d} \tilde{\alpha}_K^2 \norm[\intvl^d]{ \pderiv{T_K}{x_i}}^2 + 2  \sum_{i=1}^d \sum_{K \in \Z^d} \sum_{K' \neq K}\tilde{\alpha}_K \tilde{\alpha}_{K'} \ipmeas{ \pderiv{T_K}{x_i}}{ \pderiv{T_{K'}(x)}{x_i}}{\intvl^d} \\
		&= \sum_{i=1}^d  \sum_{K \in \Z^d} \tilde{\alpha}_K^2 \pi^2 K_i^2 \stepcounter{equation}\tag{\theequation}\label{line:f} = \pi^2 \sum_{K}\tilde{\alpha}_K^2 \norm[2]{K}^2
	\end{align*}
	
	We obtain equation \eqref{line:nnn} by applying Lemma \ref{lemma:trig-expansion-deriv}, noting that $\tilde{f}$ has periodic boundary conditions and that all partial derivatives of $\tilde{f}$ are in $\fnmeas{\intvl^d}$ because the Lipschitzness of $\tilde{f}$ mandates that 
	\[\norm[\intvl^d]{\pderiv{\tilde{f}}{x_i}} \leq \norm[\intvl^d]{\nabla \tilde{f}} \leq 2L.\]
	Equation \eqref{line:f} follows from Fact \ref{fact:trig-pderiv}. 
	An immediate consequence of the above inequality is that $\abs{\tilde{\alpha}_K} \leq \frac{2L}{\pi} \leq L$ as long as $K \neq \vec{0}$. 
	Because $\abs{\EE[\bx]{\tilde{f}(\bx)}} \leq L$, $\abs{\tilde{\alpha}_{\vec{0}}} \leq L$ as well.
	Additionally, we define the trigonometric polynomial $\tilde{P} = \sum_{K: \norm[2]{K} \leq k} \tilde{\beta}_K T_K$ by letting $\tilde{\beta}_K := \tilde{\alpha}_K$ for all $K$ with $\norm[2]{K} \leq k$. By making use of Parseval (Fact \ref{fact:parseval-plancherel}) and the inequality ending on line \eqref{line:f},
	\begin{align*}
		\norm[\intvl^d]{\tilde{f} - \tilde{P}}^2 
		&= \sum_{K: \norm[2]{K} > k} \tilde{\alpha}_K^2 
		\leq \sum_{K: \norm[2]{K} > k} \tilde{\alpha}_K^2 \cdot \frac{\norm[2]{K}^2}{k^2} 
		\leq  \frac{1}{k^2}\sum_{K \in \Z^d} \tilde{\alpha}_K^2 \norm[2]{K}^2 \\ 
		&\leq \frac{4L^2}{\pi^2 k^2} 
		\leq \frac{L^2}{ k^2} 
		\leq \eps^2, \quad \text{which establishes step~(\ref{step:3})}.
	\end{align*}
		
	For step (\ref{step:4}), if $\tilde{P}$ $\eps$-approximates $\tilde{f}$ over $\fnmeas{\intvl^d}$, then there must exist a unit cube in some orthant corresponding to some $w \in \flip^d$ where $\tilde{P}$ also $\eps$-approximates $\tilde{f}$. That is,
	\[\EE[\bx \sim \intv^d]{\paren{\tilde{P}(w \odot \bx) - \bar{f}( \bx)}^2} \leq \eps^2.\]
	
	For step (\ref{step:5}), by translating the distribution from $\intvl^d$ to $\intv^d$ and taking $P(x) := \tilde{P}\paren{\frac{1}{2} w \odot (x + \vec{1})} $, we obtain
	\begin{align*}
		\EE[\bx \sim \intvl^d]{\paren{P(\bx) - f(\bx)}^2} = \EE[\bx \sim \intv^d]{\paren{\tilde{P}(w \odot \bx) - \tilde{f}( \bx)}^2} 		
	\end{align*} 
	
	It remains to show that we can represent $P$ as a proper trigonometric polynomial with halved frequencies and bounded coefficients. 
	We do so by examining each term of the expansion of $\tilde{P}$. Fix any $K \in \Z^d$ with $\norm[2]{K} \leq k$ and $K \in \sinset$. 
	Then, $T_K(x) = \sqrt{2} \sin(\pi \innerprod{K}{x})$. 
	Consider the term corresponding to $K$ of $P(x)$ represented as an expansion of $\tilde{P}$, $\tilde{\beta}_K T_K\paren{ \half w \odot (x + \vec{1})}$. By rearranging its inner product and applying sum-of-angles trigonometric identities, we obtain the following identity:
	\begin{align*}
		T_K\paren{ \half w \odot (x + \vec{1})} 
		&= \sqrt{2}  \sin\paren{\frac{\pi}{2} \innerprod{w \odot K}{x} + \frac{\pi}{2} \innerprod{w \odot K}{\vec{1}}} \\
		&= \begin{cases}
			\sqrt{2}  \sin\paren{\frac{\pi}{2} \innerprod{w \odot K}{x} }, & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 0 \pmod 4 \\
			\sqrt{2}  \cos\paren{\frac{\pi}{2} \innerprod{w \odot K}{x} }, & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 1 \pmod 4 \\
			-\sqrt{2}  \sin\paren{\frac{\pi}{2} \innerprod{w \odot K}{x} }, & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 2 \pmod 4 \\
			-\sqrt{2}  \cos\paren{\frac{\pi}{2} \innerprod{w \odot K}{x} }, & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 3 \pmod 4 
		\end{cases}
			\end{align*}
	which yield the final representation for $T_K$ functions:
	\begin{align*}
			T_K\paren{ \half w \odot (x + \vec{1})} 
	&= \begin{cases}
			T_{w \odot K}(\half x), & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 0 \pmod 4 \\
			T_{-w \odot K}(\half x), & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 1 \pmod 4 \\
			-T_{w \odot K}(\half x), & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 2 \pmod 4 \\
			-T_{-w \odot K}(\half x), & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 3 \pmod 4 
		\end{cases}.
	\end{align*}
	
	Similarly,
	\[T_{-K}\paren{ \half w \odot (x + \vec{1})} = 
	\begin{cases}
		T_{-w \odot K}(\half x), & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 0 \pmod 4 \\
		-T_{w \odot K}(\half x), & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 1 \pmod 4 \\
		-T_{-w \odot K}(\half x), & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 2 \pmod 4 \\
		T_{w \odot K}(\half x), & \text{if }\innerprod{w \odot K}{\vec{1}} \equiv 3 \pmod 4 
	\end{cases}.\]
	
	Using these identities, we can rewrite $P$ as its own trigonometric polynomial with coefficients $\beta_K$ for all $K \in \Z^d$ such that $\beta_K \in \set{\tilde{\beta}_{w \odot K}, - \tilde{\beta}_{w \odot K}}$ if $\innerprod{w \odot K}{\vec{1}} \equiv 0 \pmod 2$, and $\beta_K \in \set{\tilde{\beta}_{-w \odot K}, - \tilde{\beta}_{-w \odot K}}$ otherwise. 
	Such $\beta_K$ exist such that the following holds, which gives a trigonometric polynomial that approximates $f$ over $[-1, 1]^d$:
	\[P(x) = \sum_{K: \norm[2]{K} \leq k} \tilde{\beta}_K T_K\paren{\frac{1}{2} w \odot (x + \vec{1})} = \sum_{K: \norm[2]{K} \leq k} \beta_K T_{K}\paren{\frac{x}{2}}.\]
		
\end{proof}

==> arxiv_commands.tex <==
%

\usepackage{xcolor}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{pgfplots}
\usepackage{xstring}
\usepackage{trimspaces}
\usepackage{thmtools}
\usepackage{thm-restate}

\usepackage{enumitem}
\setlist{leftmargin=\parindent,topsep=0.25em,partopsep=0.25em,parsep=0.25em,itemsep=0.25em}

\DeclareMathOperator{\dif}{d \!}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\poly}{poly}
\newcommand{\expectation}[2][]{\mathop{\mathbb{E}}\displaylimits_{#1}\left[ #2 \right]}
\newcommand{\EE}[2][]{\mathop{\mathbb{E}}\displaylimits_{#1}\left[ #2 \right]}
\newcommand{\EEl}[2][]{\mathop{\mathbb{E}}\displaylimits_{#1}[ #2 ]}
\newcommand{\indicator}[1]{\mathds{1}\left\{ #1 \right\}}
\newcommand{\indicatorl}[1]{\mathds{1}\{ #1 \}}
\newcommand{\Var}[2][]{\mathop{\operatorname{Var}}_{#1}\left( #2\right)}
\newcommand{\Cov}[3][]{\mathop{\operatorname{Cov}}_{#1}\left( #2, #3\right)}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\ProbE}[1]{\mathbb{P} \left[ #1 \right]}
\newcommand{\pr}[2][]{\mathop{\operatorname{Pr}}\displaylimits_{#1}\left[ #2 \right]}
\newcommand{\prl}[2][]{\mathop{\operatorname{Pr}}\displaylimits_{#1}[ #2 ]}
\newcommand{\E}[1]{\mathbb{E} \left[ #1 \right]}
\newcommand{\CurlyB}[1]{\left\{ #1 \right\}}
\newcommand{\norm}[2][]{\left\| #2 \right\|_{#1}}
\newcommand{\norml}[2][]{\| #2 \|_{#1}}
\newcommand{\normInf}[1]{\norm[\infty]{#1}}
\newcommand{\normOne}[1]{\norm[1]{#1}}
\newcommand{\innerprod}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\innerprodl}[2]{\langle #1, #2 \rangle}
\newcommand{\innerproduct}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\sign}[1]{\operatorname{sign}\left( #1 \right)}
\newcommand{\signl}[1]{\operatorname{sign}( #1 )}
\newcommand{\relu}{\sigma_{\operatorname{ReLU}}}
\newcommand{\parity}{\operatorname{Par}}
\newcommand{\re}{\operatorname{Re}}
\newcommand{\im}{\operatorname{Im}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\floorl}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\ceill}[1]{\lceil #1 \rceil}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\absl}[1]{| #1 |}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\setl}[1]{\{ #1 \}}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\parenl}[1]{( #1 )}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\bracketl}[1]{[#1]}


\newcommand{\recip}[1]{\frac{1}{#1}}

\newcommand{\eps}{\epsilon}

\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Circle}{\mathbb{T}}

\newcommand{\flip}{\{-1, 1\}}
\newcommand{\bit}{\{0, 1\}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\halfl}{\fracl{1}{2}}

\newcommand\X{{\mathcal{X}}}
\newcommand\ip[1]{\langle #1 \rangle}
\newcommand\bb{{\mathbf{b}}}
\newcommand\bbi[1]{{\mathbf{b}^{( #1 )}}}
\newcommand\bg{{\mathbf{g}}}
\newcommand\gi[1]{{{g}^{( #1 )}}}
\newcommand\bgi[1]{{\mathbf{g}^{( #1 )}}}
\newcommand\bh{{\mathbf{h}}}
\newcommand\bhi[1]{{\mathbf{h}^{( #1 )}}}
\newcommand\bu{{\mathbf{u}}}
\newcommand\bd{{\mathbf{d}}}
\newcommand\bv{{\mathbf{v}}}
\newcommand\bvi[1]{{\mathbf{v}^{( #1 )}}}
\newcommand\bw{{\mathbf{w}}}
\newcommand\wi[1]{{{w}^{( #1 )}}}
\newcommand\bwi[1]{{\mathbf{w}^{( #1 )}}}

\newcommand\bx{{\mathbf{x}}}
\newcommand\by{{\mathbf{y}}}
\newcommand\bK{{\mathbf{K}}}

\newcommand\x{{\mathbf{x}}}
\newcommand\z{{\mathbf{z}}}
\newcommand\F{\mathcal{F}}
\newcommand\T{{\scriptscriptstyle{\mathsf{T}}}}
\newcommand\Normal{\operatorname{\mathcal{N}}}
\newcommand\MNormal{\Normal(0, I_d)}
\newcommand\vol{\operatorname{vol}}

\newcommand\minwidth[5]{\operatorname{MinWidth}_{#1, #2, #3, #4, #5}}


\newcommand\sobolev[2]{H^{#1}(#2)}
\newcommand\fnmeas[1]{L_2(#1)}
\newcommand\sobnorm[3]{\norm[\sobolev{#1}{#2}]{#3}}
\newcommand\ipmeas[3]{\innerprod{#1}{#2}_{#3}}
\newcommand\ipmeasl[3]{\innerprodl{#1}{#2}_{#3}}
\newcommand\intvl{[-1, 1]}
\newcommand\intv{[0, 1]}
\newcommand\Span[1]{\operatorname{Span}\paren{#1}}
\newcommand\Spanl[1]{\operatorname{Span}(#1)}
\newcommand\betam{\beta_{\max}}
\newcommand\sph{\mathbb{S}^{d-1}}
\newcommand\unif[1]{\operatorname{Unif}\paren{#1}}

\newcommand{\brown}[1]{{\color{brown} #1}}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}
\newcommand{\violet}[1]{{\color{violet} #1}}
\newcommand{\purple}[1]{{\color{purple} #1}}
\newcommand{\gray}[1]{{\color{gray} #1}}


%
\newcommand{\green}[1]{{\color{green!70!black} #1}}

%
%
%
%
\newcommand{\cs}[1]{\red{\textsc{Clayton:} #1}}
\newcommand{\rs}[1]{\blue{\textsc{Rocco:} #1}}
\newcommand{\djh}[1]{\violet{\textsc{Daniel:} #1}}
\newcommand{\mv}[1]{\green{\textsc{Manolis:} #1}}

%
%
%
%
\newcommand{\ignore}[2][]{%
  \IfEqCase{#1}{%
    {}{}%
    {true}{}%
    {false}{#2}%
  }[\PackageError{ignore}{Undefined option to ignore: #1}{}]%
}

\newcommand{\bias}{\operatorname{bias}}
\newcommand{\weights}{\operatorname{weights}}
\newcommand{\dprod}{\mathcal{D}}
\newcommand{\dprodk}{\mathcal{D}_k}
\newcommand{\dbias}{\mathcal{D}_{\bias}}
\newcommand{\dweight}{\mathcal{D}_{\weights}}
\newcommand{\dweightk}{\mathcal{D}_{\weights, k}}

\newcommand{\supp}{\operatorname{supp}}

\renewcommand\vec\orgvec

\newcommand{\lip}{\operatorname{Lip}}

\newcommand{\deriv}[2]{\frac{d #1}{d #2}}
\newcommand{\nderiv}[3]{\frac{d^{#3} #1}{d #2^{#3}}}
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pderivl}[2]{\partial #1/\partial #2}
\newcommand{\npderiv}[3]{\frac{\partial^{#3} #1}{\partial #2^{#3}}}
\newcommand{\dderiv}[2]{D^{(#1)} #2}

\newcommand{\spangl}{\Spanl{\bgi{j}}_{j=1}^r}

\newcommand{\sinset}{\mathcal{K}_{\sin}}
\newcommand{\cosset}{\mathcal{K}_{\cos}}

\newcommand{\fracl}[2]{#1 / #2}

%
%
%
%
%

\newenvironment{proofnoqed}[1][Proof]%
{%
 \par\noindent{\bfseries\upshape #1.\ }%
}%
{}

\let\orgvec\vec
\renewcommand*{\vec}[1]{\boldsymbol{#1}}
%


==> arxiv_packages.tex <==

\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[compact]{titlesec}
\usepackage[usenames,dvipsnames]{xcolor}

%
%
\usepackage{cmap}
\usepackage[T1]{fontenc}
\usepackage{bm}
\pagestyle{plain}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amsthm}
\usepackage{dsfont}

%
\usepackage{mathtools}
\usepackage{xspace}
%

\usepackage{graphicx, ucs}

\usepackage{subcaption}
\usepackage{rotating}
\usepackage{float}
\usepackage{tikz}

\usepackage[hyphens]{url} 

     %
\usepackage{booktabs}       %
%
\usepackage{tcolorbox}
%
\usepackage{tikz} %
\usepackage{lipsum}
\usepackage{wrapfig}
\usetikzlibrary{shapes.geometric, arrows, positioning, calc, matrix}
\usepackage{tikz-3dplot}
\usetikzlibrary{3d}
\usetikzlibrary{decorations,calligraphy}

==> discussion.tex <==
\section{Discussion}
\cs{todo}

Next steps: learnability, $L_{\infty}$, smoothed worst-case weights

==> feedback.tex <==
%

\red{
\section*{General feedback to implement everywhere!}
Only remove items when they're done throughout the paper
\begin{itemize}
%
%
%
	\item Instead of saying ``$\mathbf{x} \in \mathcal{X}$,'' say ``$\mathbf{x}$ is a random variable taking values in $\mathcal{X}$.''
%
	\item We call distributions over $(b, w)$ \emph{parameter distributions} and distributions over only $w$ \emph{weight distributions} 
	\item Use the phrase ``infinite mixture'' to describe the combination of random ReLUs, not ``super-position,'' ``linear combination,'' ``expectation,'' or ``integral.'' (yay consistency)
	\item Watch out for log issues! If we have things like $O(\log(k))$, where $k$ might have $k \leq 1$, replace with $O(\log(k + 1))$.
\end{itemize}


\subsection*{Next round of edits.}
\begin{itemize}
  \item \textbf{Introduction:} Pare down introduction, especially in techniques section. Finish writing related works section. DH: Acknowledge other contributions to NN approximation (such as Maiorov papers) besides random features. Talk about Cho and Saul paper. Eliminate redundancy between subsections and avoid going into technical details more than once about related works. \textbf{Rocco will make first tightening pass. Daniel will make a second after.} \rs{I made a first pass on this.} \djh{I have made a pass on the intro, but relwork yet.}

\item \textbf{Preliminaries:} Lipschitzness section can be one line, just defining seminorm. Add a couple sentences introducing the trigonometric basis and referring to the appendix. \textbf{Daniel} \djh{I believe I have finished this.}

\item  \textbf{Upper-Bounds:} Preferred form of theorems is first brown one. Use second brown one in introduction. Eliminate definition of $k$. \textbf{Clayton} 
\cs{Finished close review. Ready to move things to the appendix during surgery :)}

\item  \textbf{Lower-Bounds:} General edits and beautification. \textbf{Manolis. Clayton will do the ``brown realignment.'' Daniel will also read closely.}

\item  \textbf{Trig Basis Appendix:} Eliminate comparators. Instead, define partition over $\Z^d$. Propagate throughout. \textbf{Clayton.}
\cs{Feeling pretty happy}

\item  \textbf{Combinatorics Appendix:} Quick review \textbf{Daniel.}
  \djh{I think I am happy with this now. Nice proof!}

\item  \textbf{Reflection UB Appendix:} Quick review. Figure beautification. \textbf{Daniel review, Manolis figure.}

\item  \textbf{Sobolev:} Create non-explicit LBs, get to same form. \textbf{Clayton.} 
\cs{done}

\item  \textbf{Gaussian:} Say something ``benign'' about Gaussian Sobolev. \textbf{Daniel} \djh{done}


\end{itemize}

}


==> gaussian-concise2.tex <==
%!TEX root = main.tex

\section{A Similar Approach for the Gaussian Measure}\label{asec-gaussian}

<<<<<<< HEAD
The techniques underlying our upper and lower bounds on approximation by depth-2 RBL networks are rather general, and can be applied in a broader range of settings than are captured by Theorems~\ref{thm:ub-cube-lipschitz-informal} and~\ref{thm:lb-cube-sine-informal}. These settings include other activation functions beyond ReLU gates \rs{are we comfortable saying this? we can definitely delete it if not} and other functions spaces beyond $\fnmeas{\intvl^d}$. In this Appendix we briefly sketch how several of the key ingredients for Theorems~\ref{thm:ub-cube-lipschitz-informal} and~\ref{thm:lb-cube-sine-informal} have analogues for depth-2 RBL ReLU networks over \emph{Gaussian space}.
\ignore{ and how results similar to Theorems~\ref{thm:ub-cube-lipschitz-informal} and~\ref{thm:lb-cube-sine-informal} can be proved over Gaussian space.
}
=======
The techniques underlying our upper and lower bounds on approximation by depth-2 RBL networks are rather general, and can be applied in a broader range of settings than are captured by Theorems~\ref{thm:ub-cube-lipschitz-informal} and~\ref{thm:lb-cube-sine-informal}. These settings include other activation functions beyond ReLU gates \rs{are we comfortable saying this? we can definitely delete it if not}\cs{I would definitely feel comfortable saying so\dots For our current upper-bounds, it would just come down to tweaking Lemma \ref{lemma:relu-univariate-representation} to show that we can represent one-dimensional function with combinations of that activation.}  and other functions spaces beyond $\fnmeas{\intvl^d}$. In this Appendix we briefly sketch how several of the key ingredients for Theorems~\ref{thm:ub-cube-lipschitz-informal} and~\ref{thm:lb-cube-sine-informal} have analogues over \emph{Gaussian space}, and how results similar to Theorems~\ref{thm:ub-cube-lipschitz-informal} and~\ref{thm:lb-cube-sine-informal} can be proved over Gaussian space.
>>>>>>> cbfdff10465367b0fc3c1996f5b34bc7bb4d9d23

\subsection{The setting and key background results.}

We consider the domain $\R^d$ endowed with the standard $d$-dimensional Gaussian measure $\MNormal$ with mean zero and identity covariance matrix. It is well known (see e.g.~Section 11.2 of \cite{odonnell14}) that the set $\{H_K\}_{K \in \N^d}$ of all \emph{multivariate normalized Hermite polynomials} is an orthonormal basis for $\fnmeas{\MNormal}$, where for $K=(k_1,\dots,k_d)$ the function $H_K$ is 
\[
H_K = \prod_{j=1}^d  h_{K_j}(x_j)
\]
where $h_i$ is the degree-$i$ normalized univariate Hermite polynomial.  These multivariate Hermite polynomials are analogous to the trigonometric basis polynomials $T_K$ that were introduced in Section~\ref{sec:trig-basis-body} for the function space $\fnmeas{\intvl^d}.$

Well known results \rs{add citation} show that partial derivatives of multivariate normalized Hermite polynomials can be conveniently expressed in terms of other multivariate normalized Hermite polynomials, very analogous to Equation~\ref{eq:deriv-of-trig}.  By combining this with a well-known recurrence relation for Hermite polynomials \rs{add citation}, it is possible to prove the following result, which is closely analogous to Lemma \ref{lemma:trig-expansion-deriv} but now for $\fnmeas{\MNormal}$ rather than $\fnmeas{\intvl^d}$:

\begin{lemma}[Term-by-Term Differentiation for Hermite Representation]\label{lemma:hermite-expansion-deriv}
	Consider some $f \in \fnmeas{\MNormal}$ and $i \in [d]$ such that $f$ is differentiable with respect to $x_i$ and $\pderiv{f}{x_i} \in  \fnmeas{\MNormal}$. Then, $f$ and its partial derivative $\pderiv{f}{x_i}$ have Hermite expansions of the form
\[
f = \sum_{K \in \N^d} \alpha_K H_K 
\quad \& \quad
\pderiv{f}{x_i} =  \sum_{K \in \N^d} \alpha_{K} \pderiv{H_{K}}{x_i}.
\]
\ignore{	
	 has a Hermite expansion for some $\alpha$:
	\[f = \sum_{K \in \N^d} \alpha_K H_K,\]
	and the Hermite expansion of $\pderiv{f}{x_i}$ is:
	\[\pderiv{f}{x_i} = \sum_{K \in \N^d} \beta_K H_K,\]
	where 
	\begin{equation}\label{line:m}
		\beta_{K } = \sqrt{K_i + 1} \alpha_{K + e_i}.
	\end{equation}
	
	It thus follows that
	\[\pderiv{f}{x_i} = \sum_{K \in \N^d} \alpha_{K} \pderiv{H_{K}}{x_i}.\]
}
\end{lemma}



\subsection{The upper bound approach.}

Recall that our positive results for depth-2 RBL ReLU approximation are proved in two stages.  In the first stage (Lemma~\ref{lemma:trig-lipschitz-approx}), we argued that any Lipschitz function over $\intvl^d$ can be approximated as a low-degree trigonometric polynomial with bounded coefficients.  In the second stage (Lemma~\ref{lemma:ub-cube-trig-bounded-degree}), we argued that low-degree trigonometric polynomials can be approximated with depth-2 RBL ReLU networks.

For the first stage, with Lemma~\ref{lemma:hermite-expansion-deriv} in hand as an analogue of Lemma \ref{lemma:trig-expansion-deriv}, it is possible to obtain an analogue of Lemma~\ref{lemma:trig-lipschitz-approx}; in the current Gaussian setting, this results shows that functions in $\fnmeas{\MNormal}$ with bounded Lipschitz constant can be approximated with low-degree Hermite polynomials.  (The argument is in fact simpler than for Lemma~\ref{lemma:trig-lipschitz-approx} because there are no issues with periodic boundary conditions, which were responsible for steps~1, 2, 4 and 5 of the outline provided at the beginning of the proof of Lemma~\ref{lemma:trig-lipschitz-approx}.)

For the second stage, some technical challenges arise because the Hermite basis functions (unlike the trigonometric polynomials defined in Section~\ref{sec:trig-basis-body}) are not ridge functions.  These challenges can be overcome using techniques from \cite{apvz} but the resulting arguments are somewhat lengthy so we omit both the arguments and detailed statements of the results they establish. \rs{I'm not 100\% thrilled about this approach to the exposition. But I'm also not really comfortable stating a result without proof.  If we don't state this result (the large-$d$ result) then it seems we shouldn't state the large-$(L/\eps)$ result based on Ji Telgarsky Xu either; there too if we don't give a proof I'm not really comfortable stating it.}


\subsection{The lower bound approach.}


==> gaussian.tex <==
%

\section{A Similar Approach for the Gaussian Measure}\label{asec-gaussian}


Here, we consider the Gaussian measure $\MNormal$ instead of the uniform measure on $\intvl^d$. Then,	
\[\ipmeas{f}{g}{\MNormal} := \int_{\R^d} f(x) g(x) \paren{2 \pi ^2}^{-d/2} \exp\paren{-\frac{\norm[2]{x}^2}{2}} dx.\]

\subsection{Hermite Polynomial Basis for $\fnmeas{\MNormal}$}\label{sssec:hermite}
\cs{this should be substantially trimmed/hand-waved}

\begin{definition}[Normalized Hermite polynomials]
	\cs{Should flesh out and cite}. Let $h_k: \R \to \R$ denote the \emph{univariate normalized Hermite polynomial} of degree $k$, which together form an orthonormal basis for $\fnmeas{\Normal(0, 1)}$
	
	For multi-index $K \in \N^d$, let $H_K: \R^d \to \R$ be the \emph{multivariate normalized Hermite polynomial} of degree $K$. The set of all of these polynomials form an orthonormal basis for $\fnmeas{\Normal(0, I_d)}$. Each one can be represented as a product of univariate normalized Hermite polynomials:
	\[H_K(x) = \prod_{j=1}^d h_j(x_j).\]
\end{definition}

The following fact will be useful in the subsequent sections.

\begin{fact}[Derivatives of Hermite Polynomials]\label{fact:hermite}
	For univariate normalized Hermite polynomial $h_k$:
	\[\deriv{h_k}{z} = \sqrt{k} h_{k-1}(z).\]
	
	Likewise, for multivariate normalized Hermite polynomial $H_{K}$:
	\[\pderiv{H_K}{x_i} = \sqrt{K_i} H_{K - e_i}(x),\]
	where $e_i \in \R^d$ is the vector with $1$ in the $i$th coordinate and $0$ everywhere else.
\end{fact}

The following is well-known recurrence for Hermite polynomials, scaled for normalized Hermite polynomials. \cs{need citation} \rs{Let's mention that this is analogous to (\ref{eq:Tk-derivatives}) in that it lets us express derivatives of basis functions in terms of other basis functions.}

\begin{fact}[Recurrence for Hermite Polynomials]\label{fact:hermite-recurrence}	
	For all $K \in \N^d$ and for all $i \in [d]$, 
	\begin{align*}
	\sqrt{K_i + 1} H_{K + e_i}(x) 
	&= x_i H_{K}(x) - \pderiv{H_{K}(x)}{x_i} \\
	&= \begin{cases}
		x_i H_{K}(x) - \sqrt{K_i} H_{K - e_i}(x) & \text{if $K_i \geq 1$} \\
		x_i H_{K}(x)  & \text{if $K_i = 0$} \\
	\end{cases}
	\end{align*}
\end{fact}

We prove a similar result to Lemma \ref{lemma:trig-expansion-deriv} to show conditions in which a Hermite expansion can be differentiated term-by-term.

\begin{lemma}[Term-by-Term Differentiation for Hermite Representation]\label{lemma:hermite-expansion-deriv}
	Consider some $f \in \fnmeas{\MNormal}$ and $i \in [d]$ such that $f$ is differentiable with respect to $x_i$ and $\pderiv{f}{x_i} \in  \fnmeas{\MNormal}$. Then, $f$ has a Hermite expansion for some $\alpha$:
	\[f = \sum_{K \in \N^d} \alpha_K H_K,\]
	and the Hermite expansion of $\pderiv{f}{x_i}$ is:
	\[\pderiv{f}{x_i} = \sum_{K \in \N^d} \beta_K H_K,\]
	where 
	\begin{equation}\label{line:m}
		\beta_{K } = \sqrt{K_i + 1} \alpha_{K + e_i}.
	\end{equation}
	
	It thus follows that
	\[\pderiv{f}{x_i} = \sum_{K \in \N^d} \alpha_{K} \pderiv{H_{K}}{x_i}.\]
\end{lemma}

\begin{proof}
Because $f, \pderiv{f}{x_i} \in  \fnmeas{\MNormal}$, there exist $\alpha$ and $\beta$ such that $f$ and $\pderiv{f}{x_i}$ are exactly represented by the expansions given in the lemma statement. It remains to show that \eqref{line:m} holds.

To do so, we consider the term $\EE[\bx]{\bx_i f(\bx) H_{K}(\bx)}$. There are two key equalities we obtain:
\begin{enumerate}
\item By Gaussian integration-by-parts \cs{cite IBP requirements from Gaussian Processes book}: 
\begin{align*}
	\EE[\bx]{\bx_i f(x) H_{K}(\bx)}
	&= \EE[\bx]{\pderiv{(f(\bx) H_K(\bx))}{\bx_i}} \\
	&= \EE[\bx]{\pderiv{f(\bx)}{\bx_i} H_{K}(\bx)} + \EE[\bx]{f(\bx) \pderiv{H_K(\bx)}{\bx_i}}
\end{align*}

To apply the Gaussian integration-by-parts result, we require the following absolute convergences:
\[\EE[\bx]{\abs{\bx_i f(\bx) H_{K}(\bx)}}, \EE[\bx]{\abs{\pderiv{f(\bx)}{\bx_i} H_{K}(\bx)}}, \EE[\bx]{\abs{f(\bx) \pderiv{H_K(\bx)}{\bx_i}}} < \infty.\]

We obtain each relationship by making use of the Cauchy-Schwarz inequality and the fact that $f$, $\pderiv{f}{\bx_i}$, and all polynomials have bounded $L_2$ norm.
\begin{align*}
	\EE[\bx]{\abs{\bx_i f(\bx) H_{K}(\bx)}}
	&\leq \norm[\MNormal]{f}^2 \EE[\bx]{\bx_i^2 H_K(\bx)^2} 
	< \infty \\
	\EE[\bx]{\abs{\pderiv{f(\bx)}{\bx_i} H_{K}(\bx)}}
	&\leq \norm[\MNormal]{\pderiv{f}{\bx_i}}^2 \norm[\MNormal]{H_K}^2
	< \infty \\
	\EE[\bx]{\abs{f(\bx) \pderiv{H_K(\bx)}{x_i}}}
	&\leq \norm[\MNormal]{f}^2 \norm[\MNormal]{\pderiv{H_K}{\bx_i}} ^2
	< \infty
\end{align*}

\item  By using Fact \ref{fact:hermite-recurrence},
\[\sqrt{K_i + 1} H_{K + e_i}(x) = x_i H_{K }(x) - \pderiv{H_{K}(x)}{x_i},\]
we have:
\[\EE[\bx]{\bx_i f(\bx) H_{K}(\bx)}  = \sqrt{K_1+ 1} \EE[\bx]{f(\bx) H_{K + e_i}(\bx)} + \EE[\bx]{f(\bx)\pderiv{H_{K}(\bx)}{\bx_i}}.\]
\end{enumerate}

By putting both sides together and using properties of orthogonality, we obtain:
\begin{align*}
\beta_{K} &= \EE[\bx]{\pderiv{f(\bx)}{\bx_i} H_{K}(\bx_i)} \\
&= \sqrt{K_i + 1} \EE[\bx]{f(\bx) H_{K + e_i}(\bx)} \\
&= \sqrt{K_i + 1} \alpha_{K + e_i}.
\end{align*}

\end{proof}

\subsection{Approximating Lipschitz Functions with Hermite Polynomials}
We give a lemma for approximating Lipschitz functions over the Gaussian measure with low-degree Hermite polynomials. This result is analogous to Lemma \ref{lemma:trig-lipschitz-approx}, which instead approximates Lipschitz functions over $\intvl^d$ with trigonometric polynomials.

\begin{lemma}[Approximating Lipschitz Functions with Low-Degree Hermite Polynomials]\label{lemma:hermite-lipschitz-poly-approx}
	Fix some $L, \eps > 0$ with $\frac{L}{\eps} \geq 1$ \cs{is this necessary? if so, is it needed elsewhere?} and consider any $f: \R^d \to \R$ with $f \in \fnmeas{\Normal(0, I_d)}$, $\norm[\lip]{f} \leq L$, and $\abs{\EE[x \sim \Normal(0, I_d)]{f(x)}} \leq L$. Then, there exists some $k$-degree polynomial \[P(x) = \sum_{\substack{K \in \mathbb{N}^d \\ \norm[1]{K} \leq k}} \beta_K H_K(x) \]
	with $\abs{\beta_K} \leq L$ for $k = \ceil{\frac{L^2}{\eps^2}}$ such that 
	\[\norm[\Normal(0, I_d)]{f - P} \leq \eps.\]
\end{lemma}
\begin{proof}
	Suppose 
	\[f(x) = \sum_{\substack{K \in \mathbb{N}^d}} \alpha_K H_K(x),\]
	where $H_K$ is a normalized multivariate Hermite polynomial of degree $K$. 
	
	Because the Lipschitz constant is an upper-bound on the norm of the gradient,
	
	\begin{align*}
		L^2 
		&\geq \EE[\bx]{\norm[2]{\nabla f(\bx)}^2}\\
		&= \sum_{i=1}^d \EE[\bx]{\paren{\pderiv{f(\bx)}{\bx_i}}^2} \\
		&= \sum_{i=1}^d \EE[\bx]{\paren{ \sum_{K \in \N^d} \alpha_{K} \pderiv{H_K(\bx)}{\bx_i}}^2} && \text{(Lemma \ref{lemma:hermite-expansion-deriv})} \\
		&= \sum_{i=1}^d \EE[\bx]{\paren{ \sum_{K \in \N^d} \alpha_{K}\sqrt{K_i} H_{K - e_i}(\bx) }^2} && \text{(Fact \ref{fact:hermite})}\\
		&= \sum_{i=1}^d \sum_{K \in \N^d}\alpha_{K}^2 K_i  && \text{(Hermite Orthonormality)}\\
		&= \sum_{K \in \N^d}\alpha_{K}^2 \norm[1]{K} 
	\end{align*}
	
	We can apply Lemma \ref{lemma:hermite-expansion-deriv} because the Lipschitzness assumption allows us to upper-bound $\abs{f}$ and $\abs{\pderiv{f}{x_i}}$ with low-degree polynomials. \cs{flesh out?}
	
	Define $P$ by letting $\beta_K := \alpha_K$ for all $K$ with $\norm[1]{K} \leq k$. By making use of Parseval (Fact \ref{fact:parseval-plancherel}) and the above chain of inequalities,
	\begin{align*}
		\norm[\Normal(0, I_d)]{f - P}^2 
		&= \sum_{K: \norm[1]{K} > k} \alpha_K^2 
		\leq \sum_{K: \norm[1]{K} > k} \alpha_K^2 \cdot \frac{\norm[1]{K}}{k} \leq \frac{1}{k} \sum_{K \in \N^d} \alpha_K^2 \norm[1]{K} \\
		&\leq \frac{L^2}{k}  
		\leq \eps^2
	\end{align*}
	
	Now, we give bounds on the coefficients $\beta_K$ of $P(x)$. Because $H_{0}(K) = 1$, $\alpha_{0} = \EE[\bx]{f(\bx)}$, so $\alpha_{0} \leq L$. For all other $K$, $\abs{\beta_K} \leq L$ is enforced by the preceding chain of inequalities.

\end{proof}


\subsection{Lower-Bounds on $\MNormal$}
\cs{Discuss generality of Randict lower-bound.}

==> notation.tex <==
\section{Notation and Variables}

Here, we give an exhaustive catalogue of variables in the paper with the goal of standardization. \textbf{Bold} lines are problematic due to inconsistency or overloading and should be resolved.

One big question: when do we bold and when do we not? Maybe all random variables are bold?

\subsection{Variables}

{\scriptsize
\begin{longtable}{|l|c|l|l|} \hline
	Quantity & Notation & Notes & Latex \\ \hline \hline
	Function to approximate (or not) & $f$ & & \\ \hline
	Generic functions on $\R^d$ & $f, g, g_1, \dots, g_r$ & & \\ \hline
	Dimension of samples & $d$ & & \\ \hline
	Approximation accuracy & $\eps$ & & \\ \hline
	Probability of failure & $\delta$ & & \\ \hline
	Width of RBL net & $r$ & & \\ \hline
	Measure over $\R^d$ & $\mu$ & & \\ \hline
	Sample in $\R^d$ & $x$ & & \\ \hline
	Variable in $\R$ & $z$ & & \\ \hline
	Coefficient of $g_i$ in $\Span{g_1, \dots, g_r}$ & $a_i$ & & \\ \hline
	Number of symmetric functions for randict & $N$ & & \\ \hline
	Symmetric functions for randict & $\varphi_1, \dots, \varphi_N$ & & \\ \hline
	Set of symmetric functions in LB & $\Phi_k$ & & \\ \hline
	Orthonormal Basis & $\mathcal{G}$ & & \\ \hline
	Trigonometric basis & $\mathcal{T}$ & & \\ \hline
	Element of $\mathcal{T}$ & $T_K$ & & \\ \hline
	\textbf{Degree of univariate trig polynomial} & $k$ & Reserve $k$ for only max degree? & \\ \hline
	Sobolev order & $s$ & & \\ \hline
	\textbf{Sampled ReLU bias} & $b, b_i \in \R$ & Commit to index? & \\ \hline
	\textbf{Sampled ReLU weight} & $w, w_i \in \R^d$ & Commit to index? & \\ \hline
	Distribution over $\R \times \R^d$ for $(b_i, w_i)$ & $\mathcal{D}$ & & \\ \hline
	$\R$ component of $\mathcal{D}$ & $\mathcal{D}_b$ & & \\ \hline
	$\R^d$ component of $\mathcal{D}$ & $\mathcal{D}_w$ & & \\ \hline
	Distribution over $\R \times \R^d$ for $(b_i, w_i)$ & $\mathcal{D}$ & & \\ \hline
	RBL network & $g$ & &  \\ \hline
	RBL ReLU coefficient & $u \in \R^r$ & & \\ \hline
	RBL constant term & $c$ & & \\ \hline
	\textbf{RBL linear term vector} & $a \in \R^d$ & Conflict with function span & \\ \hline
	Lipschitz constant & $L$ & & \\ \hline
	Max norm of degree of approximating (trig) poly & $k$ & & \\ \hline
	Specific weight distribution over $\R \times \R^d$ & $\mathcal{D}_k$ & & \\ \hline
	Max Sobolev norm for $f$ & $\gamma$ & & \\ \hline
	Set of indices ($\Z^d$ or $\N^d$) & $\mathcal{K}$ & & \\ \hline
	Function from multi-indices (e.g. $K \mapsto \norm[2]{K}$) & $\omega: \mathcal{K} \to \R$ & & \\ \hline
	UB on weighted combo of indices (Fact \ref{fact:markov}) & $C$ & & \\ \hline
	\textbf{Trig / Hermite coefficients for $f$} & $\alpha = (\alpha_K)_{K \in \mathcal{K}}$, $\beta = (\beta_K)_{K \in \mathcal{K}}$ & Bold $\alpha$? Inconsistent & \\ \hline
	Trig / Hermite polynomial & $P$ & & \\ \hline
	Trig / Hermite polynomial $P$ coefficients  & $\beta = (\beta_K)_{K \in \mathcal{K}}$ & Bold $\alpha$? & \\ \hline
	Absolute max coefficient & $\betam$ & & \textbackslash betam \\ \hline
	Bound on $\omega(K)$ & $\ell$ & &  \\ \hline
	Random variable over multi-index $K$ & $\mathbf{K}$ & & \\ \hline
	Probability distribution over multi-index $K$ & $\mathbf{p}$ & & \\ \hline
	Univariate function to approx in Lemma \ref{lemma:relu-univariate-representation} & $\phi$  &  & \\ \hline
	Univariate function for ridge $T_K$ & $\phi_K$  &  & \\ \hline
	Ridge function direction & $v$ & & \\ \hline
	Scalar factor of weights (Lemma \ref{ub-cube-trig-bounded-degree}) & $\rho$ & & \\ \hline
	ReLU weighting function & $h: \R^d \times \R \to \R$ & & \\ \hline
	Random feature for LB & $\bg, \bg_1, \dots, \bg_r$ & & \textbackslash bg \\ \hline
	\textbf{Accuracy parameter for randict} & $\alpha$ & Overloaded & \\ \hline
	Dimension of random subspace & $\bd$ & & \\ \hline
	\textbf{Orthonormal basis for $\Span{\bg_1, \dots, \bg_r}$} & $\bu_1, \dots, \bu_{\bd}$ & $u$ conflict & \\ \hline
	Permutation & $\pi, \pi_{i, j}$ & & \\ \hline
	Width of wide RBL net for Theorem \ref{thm:randict-relu} & $r'$ & & \\ \hline
	``Wider'' RBL network & $g'$ & & \\ \hline
	Binomial random variable & $Y$  &  & \\ \hline
	Univariate normalized Hermite & $h_k$ & & \\ \hline
	Multivariate normalized Hermite & $H_K$ & & \\ \hline
	Standard basis vectors $\R^d$ & $e_1, \dots, e_d$ & & \\ \hline
	\textbf{Scaling of trigonometric polynomials} & $\rho$ & conflict & \\ \hline
	\textbf{Domain for Lipschitz function} & $\mathcal{X}$ & prob unnecessary & \\ \hline
\end{longtable}
}

\subsection{Indices}
{\scriptsize
\begin{tabular}{|l|c|l|l|} \hline
	Quantity & Notation & Notes & Latex \\ \hline \hline
	Index of spanning coefficients & $i$ & & \\ \hline
	Index for symmetric randict functions & $i, j$ & & \\ \hline
	Multi-index in $\Z^d, \N^d, \mathcal{K}$ & $K, K', M$ & & \\ \hline
	\textbf{Index for RBL net width} & $i, k $ & $k$ bad & \\ \hline
	Index over sample dimension $d$ & $i, j$ & & \\ \hline
	Number of partial derivs & $p$ & & \\ \hline
	Partial deriv variable indices & $q \in [d]^p$ & &  \\ \hline
	Index for partial derivatives & $i$ & & \\ \hline
	\textbf{Univariate degree index} & $j, k, m$ & Conflict/ $k$ bad & \\ \hline
\end{tabular}
}

\subsection{Notation}
{\scriptsize
\begin{tabular}{|l|c|l|l|} \hline
	Quantity & Notation & Notes & Latex \\ \hline \hline
	Function inner-product for measure $\mu$ & $\ipmeas{\cdot}{\cdot}{\mu}$ & & \textbackslash ipmeas \\ \hline
	Function $L_2$ norm for measure $\mu$ & $\norm[\mu]{\cdot}$ & & \textbackslash norm[\textbackslash mu]\{\textbackslash cdot\} \\ \hline
	Functions with bounded $\mu$ norm & $\fnmeas{\mu}$ & & \textbackslash fnmeas \\ \hline
		Univariate Gaussian & $\Normal(0, \alpha^2)$ & & \textbackslash Normal \\ \hline
	Multivariate Gaussian & $\Normal(0, \alpha^2 I_d)$ & & \textbackslash MNormal for $\alpha = 1$ \\ \hline
	\textbf{Uniform Distribution on $[-1, 1]^d$} & $\intvl^d$, $\text{Unif}(\intvl^d)$ & Abuse of notation, Confict & \textbackslash intvl\textasciicircum d \\ \hline
	Span of functions $g_1, \dots, g_r$ &  $W = \Span{g_1, \dots, g_r}$ & &  \textbackslash Span \\ \hline
	Projection to subspace $W$ of $\fnmeas{\mu}$ & $\Pi_W$ & & \\ \hline
	Mutual coherence of $\varphi_1, \dots, \varphi_N$ & $\kappa(\varphi_1, \dots, \varphi_N)$ & & \\ \hline
	\textbf{Zero vector} & $0$ OR $\vec{0}$ & Inconsistent & \\ \hline
	$(x_2, \dots, x_d)$ & $x_{2:}$ & Consider replacing with $x_{-1}$? & \\ \hline
	Indicator & $\indicator{\cdot}$ & & \textbackslash indicator \\ \hline
	$q$ sequence of partial derivs for $f$ & $f^q$ & & \\ \hline
	Sequence of partial derivs multi-index $M$ & $f^M$ & & \\ \hline
	Functions with bounded Sobolev norm & $\sobolev{s}{\mu}$ & & \textbackslash sobolev \\ \hline
	$L_2$ $s$-order Sobolev norm & $\sobnorm{s}{\mu}{\cdot}$ & &  \textbackslash sobnorm \\ \hline
	ReLU & $\sigma_r$ & & \\ \hline
	Minimum width of approximating RBL net & $\minwidth{f}{\eps}{\delta}{\mu}{\mathcal{D}}$ & & \textbackslash minwidth \\ \hline
	$\abs{\set{K \in \Z^d: \norm[2]{K} \leq k}}$ & $Q_{k, d}$ & & \\ \hline
	Set of multi-index multiples of $w$ & $K_w$ & & \\ \hline
	Binomial distribution & $\text{Bin}(\cdot, \cdot)$ & & \\ \hline
	Probability event & $E_i$ & & \\ \hline
	Multi-index for vector of indices $q$ & $M_q$ & & \\ \hline
	$\sum_{\substack{q \in [d]^p \\ M_q \leq K}}   \frac{K!}{(K - M_q)!}$ & $N(K, p)$ & & \\ \hline
	Element-wise multiplication & $\odot$ & & \\ \hline
	Element-wise sign & $\sign{\cdot}$ & & \\ \hline
\end{tabular}
}

\subsection{Sets}
{\scriptsize
\begin{tabular}{|l|c|l|l|} \hline
	Quantity & Notation & Notes & Latex \\ \hline \hline
	Real Numbers & $\R$ & & \textbackslash R \\ \hline
	Integers & $\Z$ & & \textbackslash Z \\ \hline
	Positive Integers & $\Z^+$ & & \\ \hline
	\textbf{Non-negative Integers} & $\N$ or $\Z^{\geq 0}$ or $\Z_{\geq 0}$ & Redundant & \textbackslash N \\ \hline
	Hypersphere in $\R^d$ & $\sph$ & & \textbackslash sph \\ \hline
\end{tabular}
}

==> related_work.tex <==
%

\subsection{Related Work} \label{sec:related-work}

\cs{restructure: upper-bounds and lower-bounds are main divider. rearrange paragraphs. Daniel will check out}

\noindent {\bf Approximation with depth-two networks.}
Beyond the pioneering universal approximation results for (non-RBL) depth-2 neural networks \citep{cyb89,funahashi1989approximate,hsw89} mentioned in the introduction, several subsequent works establish quantiative upper- and lower-bounds on the width of such networks required to approximate certain classes of functions.
In this section, we focus on results that provide non-asymptotic bounds.
The survey of \citet{pinkus1999approximation} provides an overview of asymptotic rates of approximation (which regard the dimension $d$ as fixed).

A line of inquiry, starting with \cite{barron93}, investigates non-asymptotic upper-bounds on the minimum width of any (non-RBL) depth-2 network sufficient to approximate certain functions in terms of a smoothness measure defined via their Fourier transforms.
These approaches use randomization as an intermediate step: they represent the target function as a mixture of activation functions drawn from some distribution that depends on the function, and obtain a depth-two network approximating the function by sampling sufficiently many activation functions from that distribution. 
We follow a similar overall approach, but with the crucial difference that in our RBL setting, our distribution of ReLUs does not depend on the specific target function being approximated.
\footnote{\djh{I modified this to remove reference to the YS paper, since that one is for RBL nets.}}

%
%
%
%
%

We note that our upper-bounds for RBL networks approximating smooth functions of course yield upper-bounds for unconstrained depth-2 networks as well, and that to our knowledge, even those upper-bounds for unconstrained networks  approximating smooth functions are novel.\footnote{\djh{omit?}}

Turning to lower-bounds, a number of recent papers have given width lower-bounds for arbitrary (non-RBL) depth-2 networks that approximate certain types of multivariate functions.
\cite{es15} and \cite{ss16} give $\exp(d)$-type lower-bounds on the width that depth-2 networks require to $L_2$-approximate certain simple functions under certain probability measures on $\R^d.$ 
In \cite{es15} the function being approximated is not explicit, and in \cite{ss16} the lower bound is only for very high-accuracy approximation (to error at most $1/d^4$), and in both works the relevant probability measures are rather involved.
In contrast, our lower bounds hold only for depth-2 RBL networks, but they are for simple explicit functions, for large (constant) values of the approximation parameter, and for $L_2$-approximation with respect to the uniform distribution over $\intvl^d$. 
In other relevant work on depth-2 lower bounds, \cite{mcpz13} (\cite{dan17-depth}, respectively) gave $\exp(d)$ ($\exp(d \log d)$, respectively) -type width lower bounds for depth-2 networks approximating certain functions with large Lipschitz constants, but these lower-bounds require a weight bound on the top-level combining gate.
\cs{confusing parens for Daniely, rearrange}
In contrast, our RBL lower bonds have no restrictions on the weights of the top level gate.


\medskip \noindent {\bf Random feature models.}
Like the current paper, \cite{sgt18} studies the representational capabilities of networks of random ReLU features. However, their results focus on universality rather than approximation: they show that a sufficiently large linear combination of random ReLU features over  the unit ball can approximate any continuous function arbitrarily well, but \citep[like][]{cyb89,funahashi1989approximate,hsw89} this result does not give a bound on the number of random features needed for approximation.

The work of \cite{slchw20}, which analyzes limitations on the approximation abilities of two-layer networks of random ReLU activation functions, is relevant to our lower bounds.  
Their lower-bounds are independent of the width of the network; they give functions that cannot be approximated by RBL networks of \emph{any} (potentially infinite) width.
However, their lower-bounds are for an extremely strong notion of approximation, namely $L_2$ approximation over all of $\R^d$ (without any weighting by a probability distribution).



More broadly, random feature models have also been the subject of considerable study on their own merits. One motivation is their connection to kernel methods;
in particular, an influential paper of \cite{rr07} shows that many interesting families of kernel functions can be approximated using linear combinations of random feature maps. 
Recent work on the Neural Tangent Kernel (NTK), such as \cite{jgh18}, argue that training neural networks with gradient descent with small step-sizes results in a similar learning rule to the one obtained by using the kernel method with the NTK.  When the network weights are randomly initialized, then the (finite-width) NTK corresponds to a combination of randomly drawn ReLU functions.


Perhaps the works on random features which are most closely related to our own upper-bounds are the papers of \cite{apvz}, \cite{ys19}, \cite{bach2017breaking}, and \cite{jtx19}, all of which prove approximation-theoretic results by representing a target function as the expected value of weighted activation functions drawn from some distribution. 
\begin{itemize}
\item Theorem 3.1 of \cite{apvz} shows how neural networks with complex-valued weights and exponential activation functions can approximate polynomials of bounded degree (they do not consider the problem of approximating smooth functions).
Their bounds have an exponential dependence on that degree, which translates to an exponential dependence on the Lipschitz constant $L$ even if the dimension $d$ is small; in contrast, our bounds are exponential in $\min\{d,L^2/\eps^2\}$, which can be much better if $d$ is small.

\item \cite{ys19} give both upper- and lower-bounds on the width of depth-2 RBL ReLU networks (as do we), but do not consider the problem of approximating smooth functions.
Since they consider a more stringent notion of $L_\infty$-approximation (over the unit ball), the upper-bounds on network width that they establish (see their Theorems 3.3 and 3.4) are more pessimistic than ours; similar to \cite{apvz}, their bounds have an exponential dependence on the square of the degree of the polynomials that they approximate. 

\item Proposition 3 of \cite{bach2017breaking} and Theorem E.1 of \cite{jtx19} also imply (or directly give) upper-bounds on the width of depth-2 ReLU networks that approximate certain functions, and obtain these upper-bounds by expressing the target functions as mixtures of ReLUs. Similar to \cite{ys19} they consider an $L_{\infty}$ notion of approximation, and as a result obtain quantitative upper-bounds that are always exponential in the dimension $d$.
\end{itemize}


Turning to lower-bounds, our lower-bound idea of exploiting symmetry to obtain an \emph{explicit} function that is difficult to approximate was inspired by \cite{ys19}.
Our approach for non-explicit lower bounds is quite similar to Theorem 19 of \cite{kms20}, which bounds the dimension of the space of all linear combinations of feature functions; similar to the lower-bound of \cite{kms20} (but unlike \cite{ys19}), our lower-bounds hold regardless of the size of the weights used in the linear combination of the bottom-level random features.
%

Finally, we remark that while we do not consider networks of depth larger than two, our paper was in large part inspired by results from the literature on depth separation.
\cite{tel16}, \cite{es15}, \cite{dan17-depth}, and \cite{ses19} all prove lower-bounds by constructing highly oscillatory functions and showing that shallow networks must be wide in order to approximate these functions. 
These works motivated us to directly study the relationship between the Lipschitz constant of a target function and the width needed to approximate it.


\medskip


\footnote{\rs{TO DO: Somewhere in this discussion of related work, mention the Maiorov line of papers on neural network approximation - these various works on approximation that don't use random features. Also, 
An old comment of Daniel's that I wasn't sure what to do with:  \djh{I think we should combine the NTK ref with the \cite{apvz,ys19,li2018learning,daniely2017sgd} results, since they are really saying similar things (for our purposes).}}}



